Efficient Speech Translation with Pre-trained Models

When building state-of-the-art speech translation models, the need for large computational resources is a significant obstacle due to the large training data size and complex models. The availability of pre-trained models is a promising opportunity to build strong speech translation systems efficiently. In a first step, we investigate efficient strategies to build cascaded and end-to-end speech translation systems based on pre-trained models. Using this strategy, we can train and apply the models on a single GPU. While the end-to-end models show superior translation performance to cascaded ones, the application of this technology has a limitation on the need for additional end-to-end training data. In a second step, we proposed an additional similarity loss to encourage the model to generate similar hidden representations for speech and transcript. Using this technique, we can increase the data efficiency and improve the translation quality by 6 BLEU points in scenarios with limited end-to-end training data.

==> 5_results.tex <==
\section{Results}

We evaluated the cascaded model as well as the different proposed methods for the end-to-end model on the CoVoST2 dataset. In addition, we investigated how we can reduce the need for additional end-to-end training data in a second series of experiments.


\textbf{Cascaded system}
In cascaded combination, we explore the efficiency of fine-tuning each component. Firstly we experiment on initializing with parameters of the pre-trained models to provide references. Then, we fine-tune the pre-trained wav2vec2.0 and MBart50 models with speech-to-transcript and transcript-to-translation training data, respectively. We experiment with different combinations of the pre-trained and fine-tuned parameters to explore the efficiency. 

As Table \ref{tab:cascaded} shows, for the cascaded combination, fine-tuning either ASR or MT module benefits performance, but fine-tuning the MT module contributes more to speech translation compared with fine-tuning the ASR module. Fine-tuning both modules leads to the best improvements of 4.9 BLEU points compared with no fine-tuning and 3.3 BLEU points improvement on the CoVoST2 Cascaded. Besides, we observe that improvement roughly equals the sum of the gains from fine-tuning each model. In addition, we find that fine-tuning the encoder of the MT model slightly improves performance. With 25\% parameters, fine-tuning the encoder achieves 41\% improvements of fine-tuning the entire MBart50.

\begin{table*}
\centering
\caption{Experiment results for model combination and fine-tuning strategy. Cascaded represents the cascaded combination, and E2E represents the end-to-end combination. PT means the pre-trained parameters, FT means the fine-tuned parameters that are from fine-tuning the entire model. Fine-tune strategy means the efficient strategy except fine-tuning the entire mode. For E2E, \#params means the fine-tuned parameters in the second stage. We report WER score for ASR tasks and BLEU score for MT and ST tasks. The CoVoST2 results are from \cite{wang2020covost} that uses the exact same dataset as us.}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccc}

\hline
     & \multicolumn{2}{c}{Initialization} & \multicolumn{3}{c}{Fine-tune strategy} & \multicolumn{3}{c}{Evaluation task} \\
     \hline
     Experiment & ASR module & MT module & MT encoder & Adapter & \#params & ASR & MT & ST\\
     \hline
     Baseline & PT & PT & - & - & - & 29.7 & 32.5 & 16.7 \\
     FT ASR 2 & FT & PT & - & - & 315M & 22.3 & - & 18.4 \\
     FT MT 3 & PT & FT & - & - & 610M & - & 37.3 & 19.5 \\
     FT both 4 & FT & FT & - & - & 925M & - & - & \textbf{21.6} \\
     FT MT's encoder 5 & FT & PT & Yes & - & 152M & - & 36.1 & 18.7 \\
     \hline
     CoVoST2 Cascaded & - &  - &  - &  - &  - &  21.4 &  29.0 &  18.3 \\
     \hline
     E2E 1 & PT & PT & - & - & - & - & - & 0 \\
     E2E 2 & FT & PT & - & - & - & - & - & 0.5 \\
     E2E 3 & PT & FT & - & - & - & - & - & 0.1 \\
     E2E 4 & FT & PT & Yes & - & 152M & - & - & \textbf{22.8} \\
     E2E 5 & PT & PT & Yes & - & 152M & - & - & 0.4 \\
     E2E 6 & FT & FT & Yes & - & 152M & - & - & 22.0 \\
     E2E 7 & FT & PT & - & Yes & 67M & - & - & 20.9 \\
    %  E2E 8 & FT & FT & - & Yes & 67M & - & - & 16.4 \\
     \hline
     CoVoST2 E2E & - &  - &  - &  - &  - &  - &  - &  16.3 \\
     \hline
     \end{tabular}}

\label{tab:model}
% \end{adjustbox}
\end{table*}

% \begin{table}[!htb]
% \begin{minipage}{0.5\linewidth}
% \caption{Cascaded combinations for the English-German language pair. The ASR results are reported in WER, the MT and ST tasks are reported in BLEU. \#params mean how many parameters are fine-tuned.}
% \label{tab:cascaded}
% % \begin{adjustbox}{center}
% \begin{tabular}{ccccc} 
%     \toprule 
%      & ASR &MT & ST & \#params \\
%       \midrule
%       Baseline &  29.7 & 32.5 & 16.7 & - \\ 
%       FT ASR & 22.3 & - & 18.4 & 315M \\
%       FT MT & - & 37.3 & 19.5 & 610M\\
%       FT both & - & - & \textbf{21.6} & 925M \\
%       FT MT.encoder & - & 36.1 & 18.7 & 152M \\
%       CoVoST2 & 21.4 & 29.0 & 18.3 & - \\
%      \bottomrule

%  \end{tabular}
%  % \end{adjustbox}
% \end{minipage}
% \begin{minipage}{0.5\linewidth}
% \caption{End-to-end combination experiments results. ASR and MT mean the parameter initialization of the end-to-end model components. PT means pre-trained, FT means fine-tuned. Training strategy indicates which component is fine-tuned. \textit{No} means the experiment has no fine-tuning.}
% \label{tab:e2e}
% % \begin{adjustbox}{width=350pt, center}
% \begin{tabular}{cccccc} 
%     \toprule 
%      & ASR & MT & Training  & \verb|#|params & BLEU \\
%      \midrule
%     E1 & PT & PT & No & - & 0 \\ 
%     E2 & FT & PT & No & - & 0.5 \\ 
%     E3 & FT & FT & No & - & 0.1 \\ 
%     E4 & FT & PT & MT.encoder & 152M & \textbf{22.8} \\ 
%     E5 & PT & PT & MT.encoder & 152M & 0.4 \\ 
%     E6 & FT & FT & MT.encoder & 152M &22.0 \\ 
%     E7 & FT & PT & Adapt layers & 67M & \textbf{20.9} \\
%     % E8 & FT & FT & Adapt layers & 67M & 16.4\\
%     CoVoST2 & - & - & - & - & 16.3 \\
%     \bottomrule
% \end{tabular}
% \end{minipage}

% \end{table}




% \begin{table}[ht]
% \caption{Cascaded combinations for the English-German language pair. The ASR results are reported in WER, the MT and ST tasks are reported in BLEU. \#params mean how many parameters are fine-tuned.}
% \label{tab:cascaded}
% % \begin{adjustbox}{center}
% \begin{tabular}{ccccc} 
%     \toprule 
%      & ASR &MT & ST & \#params \\
%      \midrule
%      Baseline &  29.7 & 32.5 & 16.7 & - \\ 
%      Fine-tune wav2vec2.0 & 22.3 & - & 18.4 & 315M \\
%      Fine-tune MBart50 & - & 37.3 & 19.5 & 610M\\
%      Fine-tune both & - & - & \textbf{21.6} & 925M \\
%      Fine-tune MBart50.encoder & - & 36.1 & 18.7 & 152M \\
%      CoVoST2 & 21.4 & 29.0 & 18.3 & - \\
%     \bottomrule

% \end{tabular}
% % \end{adjustbox}
% \end{table}


\textbf{End-to-end system} In the end-to-end combination, we apply a two-stage training scheme. The first stage is fine-tuning the pre-trained models, and the second stage is fine-tuning the end-to-end model with the end-to-end data. The two-stage training is motivated to reduce the cost of computational resources by leveraging the available data resource as described in Section \ref{e2e}.
.

In light of building the cascaded model directly using the ASR and MT modules, we first experiment with the initialization on the end-to-end system. As Table \ref{tab:e2e} shows, the end-to-end model does not work without the end-to-end training data according to experiments 1, 2 and 3. 

Next, we experiment with the end-to-end training data on different fine-tuning modules in the first stage and fine-tuning the MT encoder or adapter in the second stage to address computation efficiency. As shown in experiments 4, 5 and 6, we find that fine-tuning the ASR module in the first stage is necessary to enable speech translation for the end-to-end combination. On the contrary, fine-tuning the MT module in the first stage barely influences speech translation performance. 

In conclusion, the two-stage approach that trains the ASR component independently in the first stage and the MT encoder using the end-to-end data in the second stage is promising to build end-to-end ST systems. With this configuration (E4), we can achieve a better translation quality than the cascaded system. Furthermore, the end-to-end combination achieves 4.5 BLEU points improvements compared with the CoVoST2 E2E.

A second approach is to integrate an additional adapt layer (E7). In this case, we only need to train 67M parameter instead of 150M ones. The final performance is 2 BLEU point worse. However, the pre-trained MT model is not changed and therefore can for example still be used to perform text translation in parallel.

% \begin{table}[ht]
% \caption{End-to-end combination experiments results. ASR and MT mean the parameter initialization of the end-to-end model components. PT means pre-trained, FT means fine-tuned. Training strategy indicates which component is fine-tuned. \textit{No} means the experiment has no fine-tuning.}
% \label{tab:e2e}
% % \begin{adjustbox}{width=350pt, center}
% \begin{tabular}{cccccc} 
%     \toprule 
%      & ASR & MT & Training  & \verb|#|params & BLEU \\
%      \midrule
%     E1 & PT & PT & No & - & 0 \\ 
%     E2 & FT & PT & No & - & 0.5 \\ 
%     E3 & FT & FT & No & - & 0.1 \\ 
%     E4 & FT & PT & MT.encoder & 152M & \textbf{22.8} \\ 
%     E5 & PT & PT & MT.encoder & 152M & 0.4 \\ 
%     E6 & FT & FT & MT.encoder & 152M &22.0 \\ 
%     E7 & FT & PT & Adapt layers & 67M & \textbf{20.9} \\
%     % E8 & FT & FT & Adapt layers & 67M & 16.4\\
%     CoVoST2 & - & - & - & - & 16.3 \\
%     \bottomrule

% \end{tabular}
% % \end{adjustbox}
% \end{table}

\textbf{Data efficiency} In a second series of experiments, we evaluated the data efficiency of the end-to-end model with respect to end-to-end training data. Therefore, we investigated the effect of the similarity loss on the best performing system using the adapt layer (E7). To use the same hyperparameters as the previous experiments in model training, we scale up the similarity loss value by 100 to make it at the same scale as the original experiments. We evaluate model performance on different portions of the training data to evaluate the data efficiency.

\begin{table}
\centering
\caption{Experiment results on the similarity loss. For similarity loss, \textit{without} means training only with the similarity loss; the following portion means, continue from the \textit{without}, training with that portion of data with the original loss. The result is reported in the BLEU score.}
\begin{tabular}{cccccc}
\hline
    Experiment & None & 10\% & 15\% & 20\% & All  \\
    \hline
    Original loss & - & 0.3 & 2.0 & 11.8 & 20.9 \\ 
    New loss-BLSTM & 0 & 1.0 & 10.7 & 17.8 & 21.6 \\
    % New loss-FCN large & 0 & 0.1 & 0.1 & 1.0 & 17.0 \\ 
    % New loss-FCN small & 0 & 0.7 & 9.4 & 10.5 & 13.4\\ 
    % small setting: 3 layer + 1024 hidden size = 3.1M params; large setting: 5 layer + 4096 hidden size = 58M params; blstm has 67M params
    \hline
\end{tabular}

\label{tab:loss}
\end{table}

%According to Table \ref{tab:model} that the fine-tuned wav2vec2 is necessary. Therefore this experiment initialized with the fine-tuned wav2vec2.0 and the pre-trained MBart50. 

%The experimental result gets compared with experiment E2E 7 in Table \ref{tab:model} that has the same initialization and fine-tuning strategy.


%The experiment firstly fine-tunes the adapter with the speech-to-transcript data pairs. 

In a first experiment, we evaluated the model on the zero-shot condition, where no end-to-end training data is available. As Table \ref{tab:loss} shows, this approach fails to enable speech translation. We observe that the translation is in the source language, although with the target forcing mechanism. Therefore we expect that involving a few end-to-end data would solve the issue.

Continue from the model trained with the similarity loss, we experiment on training with the original loss using different amounts of data. We observe that training with 10\% training data enables the model to translate into the correct target language but poorly. In the case of fine-tuning with 20\% data, adding similarity loss improves 51\% compared with that without the loss. The evaluation score reaches 17.8 BLEU points, achieving 85\% performance of the best end-to-end model. Besides, compared with the learning curve of the original loss, adding the similarity loss enables the model to fulfil speech translation tasks with less training data. The advantages of adding the similarity loss demonstrate a promising approach to improving data efficiency. In addition, we observe that with all training data, training the model with the similarity loss gains 0.7 BLEU point improvement. Therefore, we conclude that involving the similarity loss increases data efficiency and benefits to improving model performance.



